Improving Molecular Force Fields with Minimal Temporal Information

Accurate prediction of energy and forces for 3D molecular systems is one of fundamental challenges at the core of AI for Science applications. Many powerful and data-efficient neural networks predict molecular energies and forces from single atomic configurations. However, one crucial aspect of the data generation process is rarely considered while learning these models i.e. Molecular Dynamics (MD) simulation. MD simulations generate time-ordered trajectories of atomic positions that fluctuate in energy and explore regions of the potential energy surface (e.g., under standard NVE/NVT ensembles), rather than being constructed to steadily lower the potential energy toward a minimum as in geometry relaxations. This work explores a novel way to leverage MD data, when available, to improve the performance of such predictors. We introduce a novel training strategy called FRAMES, that use an auxiliary loss function for exploiting the temporal relationships within MD trajectories. Counter-intuitively, on two atomistic benchmarks and a synthetic system we observe that minimal temporal information, captured by pairs of just two consecutive frames, is often sufficient to obtain the best performance, while adding longer trajectory sequences can introduce redundancy and degrade performance. On the widely used MD17 and ISO17 benchmarks, FRAMES significantly outperforms its Equiformer baseline, achieving highly competitive results in both energy and force accuracy. Our work not only presents a novel training strategy which improves the accuracy of the model, but also provides evidence that for distilling physical priors of atomic systems, more temporal data is not always better.

==> content/4_1_oc20.tex <==
\subsection{Open Catalyst 2020 (OC20) Dataset}

\paragraph{Dataset.} We further evaluate our method on the Open Catalyst 2020 (OC20) dataset~\cite{chanussot2021open}, a large-scale benchmark for machine learning in catalysis. While the dataset supports multiple tasks, we focus on the Structure to Energy and Forces (S2EF) task, which requires predicting the potential energy and atomic forces for atomic configurations sampled from MD trajectories. This setting is significantly more challenging than MD17 due to the diversity of adsorbates and catalyst surfaces involved. We conduct our experiments on the S2EF-2M subset.

\paragraph{Implementation Details.} Unlike previous experiments where models were trained from scratch, here we investigate the efficacy of FRAMES as a \textit{fine-tuning} strategy for pre-trained models. We initialize our backbone using the official pre-trained checkpoint of EquiformerV2~\citep{equiformer_v2} (31M parameters), a state-of-the-art model on this benchmark. 
A key challenge with OC20 is that the standard dataloaders provide shuffled, independent frames. To enable our temporal auxiliary loss, we pre-processed the S2EF-2M split by sorting frames according to their trajectory and frame indices. We then sampled valid tuples ($T=2$) and triples ($T=3$) of consecutive frames to compute the FRAMES auxiliary objective. The model was then fine-tuned on these temporal batches using our combined loss function.

\begin{table}[t!]
    \centering
    \scalebox{0.85}{%
    \begin{tabular}{lcccc}
    \toprule[1.2pt]
    Model & $T$ & Energy MAE (meV)$\downarrow$ & Force MAE (meV/\AA)$\downarrow$ & Training time (GPU-hours)$\downarrow$ \\
    \midrule[1.2pt]     
    EquiformerV2 (Baseline) & $1$ & 298 & 26.24 & - \\
    EquiformerV2 + FRAMES & $2$ & \textbf{XX.XX} & \textbf{XX.XX} & XX \\
    EquiformerV2 + FRAMES & $3$ & XX.XX & XX.XX & XX \\
    \bottomrule[1.2pt]
    \end{tabular}}
    \vspace{1mm}
    \caption{Comparison on the OC20 S2EF-2M dataset. We compare the pre-trained EquiformerV2 baseline against versions fine-tuned with the FRAMES objective ($T=2$ and $T=3$). Errors are averaged over the four validation sub-splits.}
    \label{tab:oc20_s2ef_equiformer}
\end{table}

\paragraph{Main Results.} The results are summarized in Table~\ref{tab:oc20_s2ef_equiformer}. Consistent with our findings on MD17 and ISO17, fine-tuning with FRAMES ($T=2$) yields improvements in force and energy accuracy over the already strong pre-trained baseline. This result is particularly notable because it demonstrates that FRAMES can be effectively applied as a post-training refinement step, improving model performance without the prohibitive cost of training large-scale models from scratch. Furthermore, we observe the same trend regarding temporal redundancy: using just two frames ($T=2$) remains sufficient for the auxiliary task, whereas increasing the context window to three frames ($T=3$) does not provide additional benefit, reinforcing our "less is more" hypothesis even in this large-scale, fine-tuning regime.
